Lasso Guarantees for $ \beta $-Mixing Heavy Tailed Time Series

Many theoretical results for the lasso require the samples to be iid. Recent work has provided guarantees for the lasso assuming that the time series is generated by a sparse Vector Auto-Regressive (VAR) model with Gaussian innovations. Proofs of these results rely critically on the fact that the true data generating mechanism (DGM) is a finite-order Gaussian VAR. This assumption is quite brittle: linear transformations, including selecting a subset of variables, can lead to the violation of this assumption. In order to break free from such assumptions, we derive non-asymptotic inequalities for estimation error and prediction error of the lasso estimate of the best linear predictor without assuming any special parametric form of the DGM. Instead, we rely only on (strict) stationarity and geometrically decaying \b{eta}-mixing coefficients to establish error bounds for the lasso for subweibull random vectors. The class of subweibull random variables that we introduce includes subgaussian and subexponential random variables but also includes random variables with tails heavier than an exponential. We also show that, for Gaussian processes, the \b{eta}-mixing condition can be relaxed to summability of the {\alpha}-mixing coefficients. Our work provides an alternative proof of the consistency of the lasso for sparse Gaussian VAR models. But the applicability of our results extends to non-Gaussian and non-linear times series models as the examples we provide demonstrate.

==> experiments.tex <==


\section{Examples}\label{sec:experiments}
We present five examples, two involving $\alpha$-mixing Gaussian processes and three $ \beta$-mixing sub-Gaussian vectors. One set of examples (Examples~\ref{ex:GaussVAR} and~\ref{ex:misVAR}) concern applications of the results in Section~\ref{subsect:gaus}. We consider VAR models with Gaussian innovations when the model is correctly or incorrectly specified.
In another set of examples (Examples~\ref{ex:sGVAR},~\ref{ex:ARCH},~\ref{ex:sGmisVAR}), we focus on applications of results in Section \ref{subsect:subgauss}. We consider VAR models with sub-Gaussian innovations when the model is correctly or incorrectly specified. Lastly, we go beyond linear models and introduce non-linearity in the DGM. In essence, our theory of Lasso on high dimensional time series extends beyond the classical linear Gaussian settings and provides guarantees potentially in the presence of model mis-specification, non-Gaussian innovations and/or nonlinearity in the DGM. 

\subsection{Examples of Section \ref{subsect:gaus}}





\begin{exmp}[Gaussian VAR]\label{ex:GaussVAR} Transition matrix estimation in sparse stable VAR models has
been considered by several authors in recent years \citep{davis2016sparse,han2013transition,song2011large}.
The Lasso estimator is a natural choice for the problem.
 
Formally a finite order Gaussian VAR($ d $) process is defined as follows.
Consider a sequence of serially ordered random vectors $(Z_t)_{t=1}^{T+d}$, ${Z_t}\in \R^p$ that admits the following auto-regressive representation:
\begin{align}\label{eq:VAR(1)}
{Z_t} = \mt{A}_1 {Z}_{t-1}+ \dots +  \mt{A}_d {Z}_{t-d} + {\mathcal{E}}_t
\end{align}
where each $\mt{A}_k, k=1, \dots, d$ is  a sparse non-stochastic coefficient matrix in $\R^{p \times p}$ and innovations ${\mathcal{E} }_t$ are $p$-dimensional random vectors from $\mathcal{N}( \vc{0}, \Sigma_{\epsilon})$. Assume $\lmin{\Sigma_{\epsilon}}>0$ and $\lmax{\Sigma_{\epsilon}}< \infty$. 

Assume that the VAR($ d $) process is \emph{stable}; i.e. $ \mathrm{det}\bpar{\mt{I}_{p \times p}-\sum_{k=1}^{d}\mt{A}_k z^k} \neq 0,\, \forall \verti{z} \le 1 $. 
%Note that every VAR(d) process $ (Z_t) $ has an equivalent augmented VAR($ 1 $) representation $ (\tilde{Z}_t) $ where $\tilde{Z}_t \in \R^{pd}$ (see Appendix \ref{veri:VAR}). Further, if the process $ (X_t) $ is stable and the coefficient matrices $ A_1,\cdots,A_d $ are sparse then the corresponding VAR(1) process $ (\tilde{X}_t) $ is also stable and has sparse coefficient matrix.
Now,  set $X_t:=({Z}'_t,\cdots,{Z}'_{t-d+1})'$ and $Y_t :=Z_{t+d}$ for $t = 1,\ldots,T$. 

We can verify (see Appendix \ref{veri:VAR} for details) that Assumptions \ref{as:spars}--\ref{as:alphaMix} hold. Note that $\bstar = (\mt{A}_1,\ldots,\mt{A}_d)' \in \R^{dp \times p}$.
As a result, Propositions \ref{result:rhoRE} and \ref{result:rhoDB}, and thus Corollary \ref{cor:gauss} follow   and hence we have all the high probabilistic guarantees for Lasso on Example \ref{ex:GaussVAR}. This shows that out theory covers the stable Gaussian VAR models for which \cite{basu2015regularized} provided Lasso errors bounds. \\


We state the following convenient fact because it allows us to study any finite order VAR model by considering its equivalent VAR($ 1 $) representation. See Appendix \ref*{veri:VAR} for details.

\begin{fact}
Every VAR(d) process can be written in VAR($ 1 $) form (see e.g. \cite[Ch 2.1]{lutkepohl2005new}).
\end{fact}

Therefore, without loss of generality, we can consider VAR($ 1 $) model in the ensuing Examples. 
%Assume that it is a (1) \textbf{Gaussian process} and (2) can be represented as a linear regression on its own lags. \\


%
%\begin{figure}[h]
%\centering
%\includegraphics[width=0.7\linewidth]{plots/GaussianVAR}
%\caption{$ l_2 $ estimation error of transition matrix against rescaled dimenions. }
%\label{fig:GaussianVAR}
%\end{figure}
%
%From Fig. \ref{fig:GaussianVAR}, we see it fits with our theory well. \\
\end{exmp}



\begin{exmp}[Gaussian VAR with Omitted Variable]\label{ex:misVAR}
We will study OLS estimator of a VAR(1) process when there are endogenous variables omitted. This arises naturally when the underlying DGM is high-dimensional but not all variables are available/observable/measurable to the researcher to do estimation/prediction. This also happens when the researcher mis-specifies the scope of the model.

Notice that the system of the retained set of variables is no longer a finite order VAR(and thus non-Markovian). There is model mis-specification and this example serves to illustrate that our theory is applicable to models beyond the finite order VAR setting. 

Consider a VAR(1) process $ (Z_t, \Xi_t)_{t=1}^{T+1} $ such that each vector in the sequence is generated by the recursion below:
$$
(Z_t; \Xi_t) = \mt{A} (Z_{t-1}; \Xi_{t-1}) + (\mathcal{E} _{Z, t-1}; \mathcal{E} _{\Xi, t-1})
$$
where $Z_t \in \R^{p} $,  $\Xi_t \in \R $, $ \mathcal{E} _{Z, t} \in \R^{p}  $, and $\mathcal{E} _{\Xi, t} \in \R $ are partitions of the random vectors $ (Z_t, \Xi_t) $ and $ \mathcal{E}_t $ into $ p $ and $ 1 $ variables. Also,
$$
\mt{A}:= 
\bbra{
\begin{array}{cc}
\mt{A}_{ZZ} & \mt{A}_{Z\Xi} \\ 
\mt{A}_{\Xi Z} & \mt{A}_{\Xi \Xi}
\end{array}  
}
$$
is the coefficient matrix of the VAR(1) process with $\mt{A}_{Z \Xi }   $ $ 1 $-sparse, $ \mt{A}_{Z Z } $  $ p $-sparse and $ r(\mt{A})<1 $. $ \mathcal{E}_t := (\mathcal{E} _{X, t-1}; \mathcal{E} _{Z, t-1}) $ for $ t=1,\ldots,T+1$ are iid draws from a Gaussian white noise process. 

We are interested in the OLS $ 1 $-lag estimator of the system restricted to the set of variables in $ Z_t $. Recall that
$$
\bstar := \argmin_{\mt{B} \in \R ^{p\times p}} \E \bpar{  
\vertii{
Z_t - \mt{B}'Z_{t-1}
}^2_2
}
$$
 Now,  set $ X_t := Z_t $ and $ Y_t :=Z_{t+1}$ for $ t=1,\ldots,T$. It can be shown that $ (\bstar)' =\mt{A}_{Z Z }+\mt{A}_{Z \Xi } \Sigma_{\Xi Z }(0)(\Sigma_Z)^{-1} $.
We can verify that Assumptions \ref{as:spars}--\ref{as:alphaMix} hold. See Appendix \ref{veri:misVAR} for details.
As a result, Propositions \ref{result:rhoRE} and \ref{result:rhoDB}, and thus Corollary \ref{cor:gauss} follow   and hence we have all the high probabilistic guarantees for Lasso on this non-Markovian example.

%\begin{figure}
%\centering
%\includegraphics[width=0.7\linewidth]{plots/GaussainMisspecifiedVAR}
%\caption{$ l_2 $ estimation error of transition matrix against rescaled dimenions.}
%\label{fig:GaussianMisspecifiedVAR}
%\end{figure}
%Again, we see from Fig. \ref{fig:GaussianMisspecifiedVAR} that our theory is verified. \\ \\
\end{exmp}

%Next, we investigate example applications of section \ref{subsect:subgauss}.
%
%
%
%
%
%
%
%
%
%
%
% We begin with VAR model with uniform innovations, followed by estimation under model misspecification. Lastly we consider a nonlinear time series DGM, the ARCH model. 


%%%
%end Gauss ex section
%%%
\begin{figure}[H]\label{fig:Gaus}
\centering
\subfigure[Gaussian VAR]{
\includegraphics[width=80mm]{plots/GaussianVAR}
\label{fig:subfigure1}}
\quad
\subfigure[VAR with Omitted Variable]{
\includegraphics[width=80mm]{plots/GaussainMisspecifiedVAR}
\label{fig:subfigure3}}
\quad
%
\caption{Lasso Error Bounds for Examples \ref{ex:GaussVAR} and \ref{ex:misVAR}.}
\label{fig:figure}
\end{figure}
Plots in Figure~\ref{fig:Gaus} show the Lasso errors $ \vertii{\bstar -\bhat} $ on Examples \ref{ex:GaussVAR} and~\ref{ex:misVAR} with sparsity $ s \approx p $. In all cases, we plotted the error versus the rescaled sample size $ T/s\log(p) $. The curves of different dimensions $ p $ align and their shapes are in agreement with the scaling in Theorem~\ref{result:master}. It verifies our results in 　Section~\ref{subsect:gaus}.


\red{more words on how it agrees with theory}
\red{fix the plots}

\subsection{Examples of Section \ref{subsect:subgauss}}
\begin{exmp}[VAR with Sub-Gaussian Innovations]\label{ex:sGVAR}

Consider a VAR($ 1 $) model defined as in Example \ref{ex:GaussVAR} except that we replace the Gaussian white noise innovations with sub-Gaussian ones and assume $ \vertiii{\mt{A}}<1 $. 

For example, take iid random vectors from the uniform distribution; i.e. $\forall t,\,\mathcal{E}_t \overset{iid}{\sim} \U{\bbra{-\sqrt{3}, \sqrt{3}}^p} $. These $\mathcal{E}_t$ will be independent centered isotropic sub-Gaussian random vectors,
giving us we a VAR($ 1 $) model with sub-Gaussian innovations.  Now, consider a sequence $ (Z_t)_{t=1}^{T+1} $ generated according to the model. Then, each $ Z_t $ will be a mean zero sub-Gaussian random vector.

 Now,  set $ X_t := Z_t $ and $ Y_t :=Z_{t+1}$ for $ t=1,\ldots,T$. Note that $ \bstar =A' $.
 We can verify  that Assumptions \ref{as:sparse}--\ref{as:0mean} and \ref{assum:subgauss}--\ref{assum:beta} hold. See Appendix \ref{veri:VAR} for details. Therefore, Propositions~\ref{results:REsub} and \ref{result:betaDev} and Corollary \ref{cor:subgauss} follow and and hence we have all the high probabilistic guarantees for Lasso on data generated from processes beyond just the Gaussian processes. 
%
% In particular, consider a process $ (\Xi_t) $ defined by the recursion Eq. \eqref{eq:VAR(d)}. Now, we replace the Gaussian innovations with sub-Gaussian ones. For example, take i.i.d. random vectors from mixture of Gaussians; i.e. $ U_t\sim \half \mathcal{N}(0, \Sigma_1)+\half \mathcal{N}(0, \Sigma_2) $. Then, each $ U_t $ will be mean zero sub-Gaussian random vectors with some covariance $ \Sigma $. Now, let $ \mathcal{E}_t := \Sigma^{-\half} U_t $. These  $ (\mathcal{E}_t)$ will be isotropic sub-Gaussian random vectors. Take these $ (\mathcal{E}_t) $ as our innovations, we have a sub-Gaussian VAR model. Then, each $ \Xi_t $ will be mean zero sub-Gaussian random vectors. For verifications of Assumptions \ref{as:0mean}--\ref{as:sparse} and \ref{assum:subgauss-}--\ref{assum:beta}, please refer to Appendix~\ref{veri:VAR}. Therefore, Propositions~\ref{results:REsub} and \ref{result:betaDev} and Corollary \ref{cor:subgauss} follow and and hence we have all the high probabilistic guarantees for Lasso on Example \ref{ex:sGVAR}.
%Results as shown in Fig. \ref{fig:Sub-gaussianVAR} look consistent with our theory. 

%\begin{figure}
%\centering
%\includegraphics[width=0.7\linewidth]{plots/Sub-gaussianVAR}
%\caption{$ l_2 $ estimation error of transition matrix against rescaled dimenions.}
%\label{fig:Sub-gaussianVAR}
%\end{figure}

\end{exmp}

\begin{exmp}[VAR with sub-Gaussian Innovations and Omitted Variable]\label{ex:sGmisVAR}

Using the same setup as in Example \ref{ex:misVAR} except that we replace the Gaussian white noise innovations with sub-Gaussian ones  and assume that $\vertiii{\mt{A}} < 1$. 

For example, we can take iid random vectors from the uniform distribution; i.e. $\forall t,\,\mathcal{E}_t \overset{iid}{\sim} \U{\bbra{-\sqrt{3}, \sqrt{3}}^{p+1}} $. These $\mathcal{E}_t$ will be independent centered isotropic sub-Gaussian random vectors,
giving us we a VAR($ 1 $) model with sub-Gaussian innovations.  Now, consider a sequence $ (Z_t,\mathcal{E}_t)_{t=1}^{T+1} $ generated according to the model. Then, each $ (Z_t,\mathcal{E}_t) $ will be a mean zero sub-Gaussian random vector.

 Now,  set $ X_t := Z_t $ and $ Y_t :=Z_{t+1}$ for $ t=1,\ldots,T$. It can be shown that $ (\bstar)' =\mt{A}_{Z Z }+\mt{A}_{Z \Xi } \Sigma_{\Xi Z }(0)(\Sigma_Z )^{-1} $.
 We can verify  that Assumptions \ref{as:sparse}--\ref{as:0mean} and \ref{assum:subgauss}--\ref{assum:beta} hold. See Appendix \ref{veri:misVAR} for details. Therefore, Propositions~\ref{results:REsub} and \ref{result:betaDev} and Corollary \ref{cor:subgauss} follow and and hence we have all the high probabilistic guarantees for sub-Gaussian random vectors from a non-Markovian model. 
%Results (Fig. \ref{fig:Sub-gaussianMisspecifiedVAR}) look reasonable. 
%
%\begin{figure}
%\centering
%\includegraphics[width=0.7\linewidth]{plots/Sub-gaussainMisspecifiedVAR}
%\caption{$ l_2 $ estimation error of transition matrix against rescaled dimenions.}
%\label{fig:Sub-gaussianMisspecifiedVAR}
%\end{figure}

\end{exmp}



\begin{exmp}[Multivariate ARCH]\label{ex:ARCH}
%\green{Isolate the result that the best linear predictor is the submatrix of the transition matrix?}
We will explore the generality of our theory by considering a multivariate nonlinear time series model with sub-Gaussian innovations. A popular nonlinear multivariate time series model in econometrics and finance is the vector autoregressive conditionally heteroscedastic (ARCH) model. Consider the following specific example of  vector ARCH model. Let $ (Z_t)_{t=1}^{T+1} $ be random vectors  defined by the following recursion, for any constants $ c>0 $, $ m\in (0,1) $, $a > 0$, and $ \mt{A} $ sparse
with $\vertiii{\mt{A}} < 1$:
\begin{align} 
\begin{split} \label{eq:ARCH}
Z_t&= \mt{A} Z_{t-1}+\Sigma(Z_{t-1}) \mathcal{E}_t \\
\Sigma(\vc{z}) &:= c \cdot \clip{\vertii{\vc{z}}^{m}}{a}{b}\mt{I}_{p \times p}
\end{split}
\end{align}
where $ \mathcal{E}_t    $ are iid random vectors from some sub-Gaussian distribution and $\clip{x}{a}{b}$ clips the argument $x$ to stay in the interval $[a,b]$. We can take innovations to be iid random vectors from uniform distribution; i.e. $\mathcal{E}_t \overset{iid}{\sim} \U{\bbra{-\sqrt{3},\sqrt{3}}^p}$ for every $ t=1,\cdots, T+1 $. Then, each $\mathcal{E}_t$ will be a mean zero isotropic sub-Gaussian random vector,
giving us we an ARCH model with sub-Gaussian innovations. Also, each $ Z_t $ will be a mean zero sub-Gaussian random vector.

 We can verify (see Appendix \ref{veri:ARCH} for details) that Assumptions \ref{as:sparse}--\ref{as:0mean} and \ref{assum:subgauss}--\ref{assum:beta} hold. In particular, note that $ \bstar $ is precisely the transpose $\mt{A}'$ of the coefficient matrix $ \mt{A} $ here, thus sparsity is built in by construction. Now,  set $ X_t := Z_t $ and $ Y_t =Z_{t+1}$ for $ t=1,\ldots,T$. Therefore, Propositions~\ref{results:REsub} and \ref{result:betaDev} and Corollary \ref{cor:subgauss} follow and and hence we have all the high probabilistic guarantees for Lasso on nonlinear models with sub-Gaussian innovations. 

\begin{figure}[H]  \label{fig:subG}
\centering
\subfigure[VAR with Sub-Gaussian Innovations]{
\includegraphics[width=60mm]{plots/Sub-gaussianVAR}
\label{fig:subfigure1}}
\quad
\subfigure[Sub-Gaussian VAR with Omitted Variable]{
\includegraphics[width=60mm]{plots/Sub-gaussainMisspecifiedVAR}
\label{fig:subfigure2}}
\subfigure[Multivariate ARCH]{
\includegraphics[width=60mm]{plots/MultivariateARCH}
\label{fig:subfigure3}}
\quad
%
\caption{Lasso Error Bounds for Examples \ref{ex:sGVAR}, \ref{ex:sGmisVAR} and \ref{ex:ARCH}.}
\label{fig:figure}
\end{figure}

Plots in Figure~\ref{fig:subG} show the Lasso errors $ \vertii{\bstar -\bhat} $ on Examples \ref{ex:sGVAR}, ~\ref{ex:sGmisVAR} and~\ref{ex:ARCH} with sparsity $ s \approx p $. In all cases, we plotted the error versus the rescaled sample size $ T/s\log(p) $. The curves of different dimensions $ p $ align and their shapes are in agreement with the scaling in Theorem~\ref{result:master}. It verifies our results in 　Section~\ref{subsect:subgauss}.
%\begin{figure}
%\centering
%\includegraphics[width=0.7\linewidth]{plots/MultivariateARCH}
%\caption{$ l_2 $ estimation error of transition matrix against rescaled dimenions.}
%\label{fig:MultivariateARCH}
%\end{figure}
%
%We see from Fig. \ref{fig:MultivariateARCH} that the lasso estimates behave exactly as theory predicts even in nonlinear model!
\end{exmp}

From plots \red{\todo{insert plots here}}, we can see that the Lasso error bounds agree with the theoretical guarantees presented in Section \ref{subsect:gaus}.

\red{more words on how it agrees with theory}

==> more_examples.tex <==



\begin{exmp}[VAR with sub-Gaussian Innovations and Misspecification]\label{ex:sGmisVAR}

Using the same setup as in Example \ref{ex:misVAR} except that we replace the Gaussian white noise innovations with sub-Gaussian ones  and assume that $\vertiii{A} < 1$. 

For example, take iid random vectors from mixture of Gaussians; i.e. $U_t\sim \half \mathcal{N}(0, \Sigma_1)+\half \mathcal{N}(0, \Sigma_2) $. Then, each $U_t$ will be a mean zero sub-Gaussian random vector with some covariance $ \Sigma $.
Now, let $ \mathcal{E}_t := \Sigma^{-\half} U_t $. These $\mathcal{E}_t$ will be centered isotropic sub-Gaussian random vectors,
giving us we a VAR($ 1 $) model with sub-Gaussian innovations. Now, consider a sequence $ (Z_t)_{t=1}^{T+1} $ generated according to the model. Then, each $ Z_t $ will be a mean zero sub-Gaussian random vector.

 Now,  set $ X_t := Z_t $ and $ Y_t :=Z_{t+1}$ for $ t=1,\ldots,T$. It can be shown that $ \bstar =(A_{Z Z }+A_{Z \Xi } \Sigma_{\Xi Z }(0)(\Sigma_Z (0))^{-1})' $.
 We can verify  that Assumptions \ref{as:sparse}--\ref{as:0mean} and \ref{assum:subgauss}--\ref{assum:beta} hold. See Appendix \ref{veri:misVAR} for details. Therefore, Propositions~\ref{results:REsub} and \ref{result:betaDev} and Corollary \ref{cor:subgauss} follow and and hence we have all the high probabilistic guarantees for Lasso on models with mis-specifications. 
%Results (Fig. \ref{fig:Sub-gaussianMisspecifiedVAR}) look reasonable. 
%
%\begin{figure}
%\centering
%\includegraphics[width=0.7\linewidth]{plots/Sub-gaussainMisspecifiedVAR}
%\caption{$ l_2 $ estimation error of transition matrix against rescaled dimenions.}
%\label{fig:Sub-gaussianMisspecifiedVAR}
%\end{figure}

\end{exmp}



==> subWeibullVAR.tex <==


All the Assumptions except for \ref{assump:subW} can be verified as in Appendix~\ref{veri:VAR}. It suffices to check Assumption~\ref{assump:subW}

Let $ \gamma $ be the parameter associated with $ (\mathcal{E}_t)$. 
 
%By recursive nature of the time series,
%\begin{align*}
%\norm[Z_t]{\psi_\gamma} \le \vertiii{A} \norm[Z_{t-1}]{\psi_\gamma} +  \norm[\mathcal{E}_{t}]{\psi_\gamma}
%\end{align*}
%which yields
%\begin{align*}
%\norm[Z_t]{\psi_\gamma} \le \frac{\norm[\mathcal{E}_{t}]{\psi_\gamma}}{1- \vertiii{A}} <\infty
%\end{align*}



Assume that the spectral radius of $ A $ is smaller than $ 1 $; i.e. $ r(A) < 1 $. This is an equivalent notion of stability of VAR process. Note that if we instead require $ \vertiii{A}<1 $, it will be a much more stringent condition, and is in fact vacuous for VAR(d), where $ d>1 $ (see for example~\cite{basu2015regularized}).

By the defintion of the spectral radius,
$$ \lim\limits_{m \to \infty}  \vertiii{A^m}^{1/m} = r(A)<1$$ In other words, there exists a positive integer $ k <\infty $ such that $  \vertiii{A^k}<1 $.

By the recursive nature of the time series,
\begin{align*}
\norm[Z_t]{\gamma_2} \le \vertiii{A^k} \norm[Z_{t-1}]{\gamma_2} +  \sum_{i=1}^{k}\vertiii{A^{k-i}}\norm[\mathcal{E}_{t-k+i}]{\gamma_2}
\end{align*}
To simplify notation, let $ C_i := \vertiii{A^{k-i}} $. Using stationarity, we have the following
\begin{align*}
\norm[Z_t]{\psi_\gamma} \le \frac{\knorm{\epsilon_t}}{1-\vertiii{A^k}} \bpar{\sum_{i=1}^{k}c_i} < \infty
\end{align*}
The last inequality follows because $ C_i<\infty, \, \forall i=1, \cdots, k$. 


Thus, the sequence $ (Z_t) $ satisfies Assumption~\ref{assump:subW}.
% with parameter $ \gamma $ given by $  \gamma = \bpar{\frac{1}{\gamma_1}+\frac{1}{\gamma_2}}^{-1} $.


==> subgaussian-beta.tex <==
\section{Sub-Gaussian Random Vectors under $\beta$-Mixing}\label{sect:subgauss}
We now focus on sub-Gaussian random vectors and present high probabilistic bounds with all parameter dependences exploit. 

\begin{assump}[Sub-Gaussianity]\label{assum:subgauss}
The sub-gaussian constants of $X_t$ and $Y_t$ are bounded above by $\sqrt{K_X}$ and $\sqrt{K_Y}$ respectively.
\end{assump}

For sub-Gaussian random vectors, we are unable to provide guarantees for Lasso just assuming $\alpha$-mixing. So we assume the stronger $\beta$-mixing condition.

\begin{assump}[$\beta$-Mixing]\label{assum:beta}
The process $\left((X_t, Y_t)\right)_{t}$ is geometrically $\beta$-mixing, i.e., there exists some constant $ c_{\beta}>0 $ such that $ \beta(l) \allowdisplaybreaks \le \allowdisplaybreaks \exp(-c_\beta l),\, $

$\forall l\ge 1  $. 
%\mid \beta_k \le c\gamma^k,\, \forall k\ge 1$ for some positive const $c$). 
\end{assump}


The stronger $\beta$-mixing condition allows us to apply the independent block technique developed by \cite{yu1994rates}. For examples of large classes of Markov and hidden Markov processes that are geometrically
$\beta$-mixing, see Theorem 3.11 and Theorem 3.12 of \cite{vidyasagar2003learning}.
In the independent blocking technique, we construct a new set of \emph{independent} blocks such that each block has the same distribution as that of the corresponding block from the original sequence. Results of~\cite{yu1994rates} provide upper bounds on the difference between probabilities of events defined using the independent blocks versus the same event defined using the original data. Classical probability theory tools for independent data can then be applied on the constructed independent blocks. In Appendix~\ref{sec:subgaussproofs}, we apply the independent blocking technique to Bernstein's inequality to get the following concentration inequality for $\beta$-mixing random variables.

\begin{lm}[Concentration of $\beta$-Mixing Sub-Gaussian Random Variables] \label{result: subgau:tailbdd}
Let ${Z} = (Z_1,\ldots,Z_T)$ consist of a sequence of mean-zero random variables with exponentially decaying $\beta$-mixing coefficients as in~\ref{assum:beta}. Let $K$ be such that $\max_{t=1}^T \snorm{Z_t} \le \sqrt{K}$. Choose a block length $a_T \ge 1$ and let $\mu_T = \lfloor T/(2a_T) \rfloor$. We have, for any $t>0 $,
\begin{align*}
\mathbb{P}[ \frac{1}{T} \vert  \Vert{Z}\Vert^2_2 - \mathbb{E}[\Vert {Z}\Vert^2_2] \vert >t ]
\le  &
4 \exp \bpar{  -C_B\min\bcur{ \frac{t^2 \mu_T}{K^2}, \frac{t \mu_T}{K}  }   } \\
  &+ 2(\mu_{T}-1) \exp\left( -c_{\beta} a_T\right)
  +
    \exp\left(\frac{- 2 t \mu_T}{K}  \right).
\end{align*}
In particular, for $0<t<K$,
\begin{align*}
\mathbb{P} \bbra{ \frac{1}{T} \vert  \Vert {Z}\Vert^2_2 - \mathbb{E}[\Vert {Z}\Vert^2_2]  \vert 
>
t
}  
\le &
4 \exp\bpar{ -C_B \frac{t^2 \mu_T}{K^2}} \\
&+
2(\mu_T-1) \exp\left( -c_{\beta} a_T\right)
+
\exp\left(\frac{- 2 t \mu_T}{K}  \right).
\end{align*}
Here $C_B$ is the universal constant appearing in Bernstein's inequality (Proposition~\ref{thm:Bernstein}).
\end{lm}

\begin{rem}
The three terms in the bound above all have interpretations: the first is a concentration term with a rate that depends on the ``effective sample size" $\mu_T$, the number of blocks; the second
is a dependence penalty accounting for the fact that the blocks are not exactly independent; and the third is a remainder term coming from the fact that $2a_T$ may not exactly divide $T$. The key terms are the first two
and exhibit a natural trade-off: increasing $a_T$ worsens the first term since $\mu_T$ decreases, but it improves the second term since there is less dependence at larger lags.
\end{rem}

\subsection{High Probability Guarantee for Lower Restricted Eigenvalue}
\begin{pr}[RE, Sub-Gaussian Case]\label{results:REsub}
Suppose Assumptions~\ref{as:stat}--\ref{as:0mean} and \ref{assum:subgauss}--\ref{assum:beta} hold.
%Consider a sequence of  stationary, $\beta$-mixing sub-Gaussian random vectors $\{X_t\}_{t=1}^T$, $X_t\in\R^p$ with sub-Gaussian constant $\sqrt{K}$, covariance matrix $\Sigma_X(0):=\mathbb{E}X_1X_1'$, and that it is geometrically ergodic, i.e. $\exists c_{\beta} >0  \mid \,\beta_k(\{X_t\}_{t=1}^T) \le \exp\{-c_{\beta}k\}$. \\
Let $C_B$ be the Berstein's inequality constant,
$\csub=\min\{C_B, 2\}$,
$b = \min\{\tfrac{1}{54K_X}\lmin{\Sigma_X},1  \}$ and
$c = \tfrac{1}{6}\max\{c_{\beta},\csub b^2\}$.
Then for
%\red{$T\ge \sqrt[\xi]{\frac{4\log{p}}{c}}$}, 
{$T \ge  \bpar{\frac{1}{c}\log(p)}^{2}$}, with probability at least
$$
1- 
  5\exp \bpar{  -\csub T^{\frac{1}{2}}  }
  -
  2(T^{\frac{1}{2}}-1)\exp \bpar{
  -c_{\beta}T^{\frac{1}{2}} 
    },
$$ we have for every vector $\vc{v} \in \R^p$,
$$
\vc{v}'  \hat{\Gamma}   \vc{v}
\ge
\alpha_2\vertii{\vc{v}}^2 
- 
\tau_2(T,p)
\vertii{\vc{v}}_1^2 ,
$$
where
\begin{align*}
\alpha_2&=\half \lmin{\Sigma_X} ,
&
\tau_2(T,p)&=\frac{27bK_X\log(p)}{c  T^\half} .
\end{align*}
\end{pr}






\subsection{High Probability Guarantee for Deviation Bound} 




\begin{pr}[Deviation Bound, Sub-Gaussian Case]\label{result:betaDev}
Suppose Assumptions \ref{as:stat}--\ref{as:0mean} and \ref{assum:subgauss}--\ref{assum:beta} hold.
Let $K = \sqrt{K_Y} + \sqrt{K_X}\bpar{1+\vertiii{\bstar} }$ and $\xi \in (0,1)$ be a free parameter. Then, for sample size
$$
T\ge \max \bcur{
\bpar{ \log(pq)  \max\bcur{ \frac{K^4}{2C_B},K^2 } }^{\frac{1}{1-\xi}},
\bbra{\frac{2}{c_{\beta}}\log(pq)   }^\frac{1}{\xi} 
},
$$
we have
\begin{align*}
\mathbb{P} &
\bbra{ \frac{1}{T} \vertiii{\mt{X}'\mt{W}}_{\infty} 
\le 
 \mathbb{Q}(\mt{X},\mt{W},\bstar)  \mathbb{R}(p,q,T) 
} \\
&\quad \quad \ge  1 -
15\exp\bpar{ - \half \log(pq)} 
 -
6(T^{1-\xi}-1) \exp\bpar{-\half c_{\beta}T^{\xi}  }
\end{align*}
where
\begin{align*}
 \mathbb{Q}(\mt{X},\mt{W},\bstar)  &=\sqrt{\frac{2K^4}{C_B}}  ,
 &
 \mathbb{R}(p,q,T) &= \sqrt{\frac{\log(pq)}{T^{1-\xi}}} .
\end{align*}
\end{pr}

\begin{rem}
Since $\xi\in (0,1)$ is a free parameter, we choose it to be arbitrarily close to zero so that $\mathbb{R}(p,q,T)$ scales at a rate arbitrarily close to $\sqrt{\frac{\log(pq)}{T}}$. However, there is a price to pay
for this: both the initial sample threshold and the success probability worsen as we make $\xi$ very small.
\end{rem}


\subsection{Putting Everything Together}

\begin{cor}[Lasso Guarantee for Sub-Gaussian Vectors under $\beta$-Mixing]
\label{cor:subgauss}
Suppose Assumptions \ref{as:spars}--\ref{as:0mean} and~\ref{assum:subgauss}--\ref{assum:beta} hold. Let $C_B,\csub,c,b$ and $K$ be as defined in Propositions \ref{results:REsub} and \ref{result:betaDev}. Let $ \xi\in(0,1)$ be a free parameter. Then, for sample size
\begin{align*}
\begin{split}
T\ge &
\max 
\left\{
 \bpar{\frac{\log(p)}{c}}^2 \max\bcur{\bpar{ \frac{1728sbK_X }{\lmin{\Sigma_{{X}}}} }^2,1 } 
, \right. \\
&\quad \qquad\left.
\bpar{ \log(pq)  \max\bcur{ \frac{K^4}{2C_B},K^2 } }^{\frac{1}{1-\xi}},
\bbra{\frac{2}{c_{\beta}}\log(pq)   }^\frac{1}{\xi} 
\right\}
\end{split}
\end{align*}
we have with probability at least
\begin{align*}
1-
15&\exp\bpar{ - \half \log(pq)} 
-
6(T^{1-\xi}-1) \exp\bpar{-\half c_{\beta}T^{\xi}  } \\
&-
 5\exp \bpar{ -\csub T^{\frac{1}{2}}  }
  -
  2(T^{\frac{1}{2}}-1)\exp \bpar{
  -c_{\beta}T^{\frac{1}{2}}
    }
\end{align*}
the Lasso error bounds~\eqref{eq:l2errorBdd} and \eqref{eq:predErrBdd} hold with
\begin{align*}
\alpha &=\half \lmin{\Sigma_X}  ,\\
\lambda_T &= 4 \mathbb{Q}(\mt{X},\mt{W},\bstar) \mathbb{R}(p,q,T)
\end{align*}
where
\begin{align*}
 \mathbb{Q}(\mt{X},\mt{W},\bstar)  &=\sqrt{\frac{2K^4}{C_B}}  ,
 &
 \mathbb{R}(p,q,T) &= \sqrt{\frac{\log(pq)}{T^{1-\xi}}} .
\end{align*}
\end{cor}

Comparing this result to the Gaussian case (Corollary~\ref{cor:gauss}), we see that the role of the condition number $\lmax{\Sigma_X}/\lmin{\Sigma_X}$ is replaced by $K_X/\lmin{\Sigma_X}$ that now serves as the ``effective condition number".

\begin{exmp}[VAR with Sub-Gaussian Innovations]\label{ex:sGVAR}

Consider a VAR($ 1 $) model defined as in Example \ref{ex:GaussVAR} except that we replace the Gaussian white noise innovations with sub-Gaussian ones and assume $ \vertiii{\mt{A}}<1 $. 

For example, take iid random vectors from the uniform distribution; i.e. $\forall t,\,\mathcal{E}_t \overset{iid}{\sim} \U{\bbra{-\sqrt{3}, \sqrt{3}}^p} $. These $\mathcal{E}_t$ will be independent centered isotropic sub-Gaussian random vectors,
giving us we a VAR($ 1 $) model with sub-Gaussian innovations.  Now, consider a sequence $ (Z_t)_{t=1}^{T+1} $ generated according to the model. Then, each $ Z_t $ will be a mean zero sub-Gaussian random vector.

 Now,  set $ X_t := Z_t $ and $ Y_t :=Z_{t+1}$ for $ t=1,\ldots,T$. Note that $ \bstar =A' $.
 We can verify  that Assumptions \ref{as:sparse}--\ref{as:0mean} and \ref{assum:subgauss}--\ref{assum:beta} hold. See Appendix \ref{veri:VAR} for details. Therefore, Propositions~\ref{results:REsub} and \ref{result:betaDev} and Corollary \ref{cor:subgauss} follow and and hence we have all the high probabilistic guarantees for Lasso on data generated from processes beyond just the Gaussian processes. 
%
% In particular, consider a process $ (\Xi_t) $ defined by the recursion Eq. \eqref{eq:VAR(d)}. Now, we replace the Gaussian innovations with sub-Gaussian ones. For example, take i.i.d. random vectors from mixture of Gaussians; i.e. $ U_t\sim \half \mathcal{N}(0, \Sigma_1)+\half \mathcal{N}(0, \Sigma_2) $. Then, each $ U_t $ will be mean zero sub-Gaussian random vectors with some covariance $ \Sigma $. Now, let $ \mathcal{E}_t := \Sigma^{-\half} U_t $. These  $ (\mathcal{E}_t)$ will be isotropic sub-Gaussian random vectors. Take these $ (\mathcal{E}_t) $ as our innovations, we have a sub-Gaussian VAR model. Then, each $ \Xi_t $ will be mean zero sub-Gaussian random vectors. For verifications of Assumptions \ref{as:0mean}--\ref{as:sparse} and \ref{assum:subgauss-}--\ref{assum:beta}, please refer to Appendix~\ref{veri:VAR}. Therefore, Propositions~\ref{results:REsub} and \ref{result:betaDev} and Corollary \ref{cor:subgauss} follow and and hence we have all the high probabilistic guarantees for Lasso on Example \ref{ex:sGVAR}.
%Results as shown in Fig. \ref{fig:Sub-gaussianVAR} look consistent with our theory. 

%\begin{figure}
%\centering
%\includegraphics[width=0.7\linewidth]{plots/Sub-gaussianVAR}
%\caption{$ l_2 $ estimation error of transition matrix against rescaled dimenions.}
%\label{fig:Sub-gaussianVAR}
%\end{figure}

\end{exmp}

\begin{exmp}[VAR with sub-Gaussian Innovations and Omitted Variable]\label{ex:sGmisVAR}

Using the same setup as in Example \ref{ex:misVAR} except that we replace the Gaussian white noise innovations with sub-Gaussian ones  and assume that $\vertiii{\mt{A}} < 1$. 

For example, we can take iid random vectors from the uniform distribution; i.e. $\forall t,\,\mathcal{E}_t \overset{iid}{\sim} \U{\bbra{-\sqrt{3}, \sqrt{3}}^{p+1}} $. These $\mathcal{E}_t$ will be independent centered isotropic sub-Gaussian random vectors,
giving us we a VAR($ 1 $) model with sub-Gaussian innovations.  Now, consider a sequence $ (Z_t,\mathcal{E}_t)_{t=1}^{T+1} $ generated according to the model. Then, each $ (Z_t,\mathcal{E}_t) $ will be a mean zero sub-Gaussian random vector.

 Now,  set $ X_t := Z_t $ and $ Y_t :=Z_{t+1}$ for $ t=1,\ldots,T$. It can be shown that $ (\bstar)' =\mt{A}_{Z Z }+\mt{A}_{Z \Xi } \Sigma_{\Xi Z }(0)(\Sigma_Z )^{-1} $.
 We can verify  that Assumptions \ref{as:sparse}--\ref{as:0mean} and \ref{assum:subgauss}--\ref{assum:beta} hold. See Appendix \ref{veri:misVAR} for details. Therefore, Propositions~\ref{results:REsub} and \ref{result:betaDev} and Corollary \ref{cor:subgauss} follow and and hence we have all the high probabilistic guarantees for sub-Gaussian random vectors from a non-Markovian model. 
%Results (Fig. \ref{fig:Sub-gaussianMisspecifiedVAR}) look reasonable. 
%
%\begin{figure}
%\centering
%\includegraphics[width=0.7\linewidth]{plots/Sub-gaussainMisspecifiedVAR}
%\caption{$ l_2 $ estimation error of transition matrix against rescaled dimenions.}
%\label{fig:Sub-gaussianMisspecifiedVAR}
%\end{figure}

\end{exmp}



\begin{exmp}[Multivariate ARCH]\label{ex:ARCH}
%\green{Isolate the result that the best linear predictor is the submatrix of the transition matrix?}
We will explore the generality of our theory by considering a multivariate nonlinear time series model with sub-Gaussian innovations. \red{Please check the following added sentence} The specification of this ARCH model is just for easy validation of  geometric $ \beta $-mixing property of the process; it may potentially be applicable to a larger class of multivariate ARCH models. A popular nonlinear multivariate time series model in econometrics and finance is the vector autoregressive conditionally heteroscedastic (ARCH) model. Consider the following specific example of  vector ARCH model. Let $ (Z_t)_{t=1}^{T+1} $ be random vectors  defined by the following recursion, for any constants $ c>0 $, $ m\in (0,1) $, $a > 0$, and $ \mt{A} $ sparse
with $\vertiii{\mt{A}} < 1$:
\begin{align} 
\begin{split} \label{eq:ARCH}
Z_t&= \mt{A} Z_{t-1}+\Sigma(Z_{t-1}) \mathcal{E}_t \\
\Sigma(\vc{z}) &:= c \cdot \clip{\vertii{\vc{z}}^{m}}{a}{b}\mt{I}_{p \times p}
\end{split}
\end{align}
where $ \mathcal{E}_t    $ are iid random vectors from some sub-Gaussian distribution and $\clip{x}{a}{b}$ clips the argument $x$ to stay in the interval $[a,b]$. We can take innovations to be iid random vectors from uniform distribution; i.e. $\mathcal{E}_t \overset{iid}{\sim} \U{\bbra{-\sqrt{3},\sqrt{3}}^p}$ for every $ t=1,\cdots, T+1 $. Then, each $\mathcal{E}_t$ will be a mean zero isotropic sub-Gaussian random vector,
giving us we an ARCH model with sub-Gaussian innovations. Also, each $ Z_t $ will be a mean zero sub-Gaussian random vector.

 We can verify (see Appendix \ref{veri:ARCH} for details) that Assumptions \ref{as:sparse}--\ref{as:0mean} and \ref{assum:subgauss}--\ref{assum:beta} hold. In particular, note that $ \bstar $ is precisely the transpose $\mt{A}'$ of the coefficient matrix $ \mt{A} $ here, thus sparsity is built in by construction. Now,  set $ X_t := Z_t $ and $ Y_t =Z_{t+1}$ for $ t=1,\ldots,T$. Therefore, Propositions~\ref{results:REsub} and \ref{result:betaDev} and Corollary \ref{cor:subgauss} follow and and hence we have all the high probabilistic guarantees for Lasso on nonlinear models with sub-Gaussian innovations. 

%\begin{figure}[H]  \label{fig:subG}
%\centering
%\subfigure[VAR with Sub-Gaussian Innovations]{
%\includegraphics[width=60mm]{plots/Sub-gaussianVAR}
%\label{fig:subfigure1}}
%\quad
%\subfigure[Sub-Gaussian VAR with Omitted Variable]{
%\includegraphics[width=60mm]{plots/Sub-gaussainMisspecifiedVAR}
%\label{fig:subfigure2}}
%\subfigure[Multivariate ARCH]{
%\includegraphics[width=60mm]{plots/MultivariateARCH}
%\label{fig:subfigure3}}
%\quad
%%
%\caption{Lasso Error Bounds for Examples \ref{ex:sGVAR}, \ref{ex:sGmisVAR} and \ref{ex:ARCH}.}
%\label{fig:figure}
%\end{figure}
%
%Plots in Figure~\ref{fig:subG} show the Lasso errors $ \vertii{\bstar -\bhat} $ on Examples \ref{ex:sGVAR}, ~\ref{ex:sGmisVAR} and~\ref{ex:ARCH} with sparsity $ s \approx p $. In all cases, we plotted the error versus the rescaled sample size $ T/s\log(p) $. The curves of different dimensions $ p $ align and their shapes are in agreement with the scaling in Theorem~\ref{result:master}. It verifies our results in 　Section~\ref{subsect:subgauss}.
%\begin{figure}
%\centering
%\includegraphics[width=0.7\linewidth]{plots/MultivariateARCH}
%\caption{$ l_2 $ estimation error of transition matrix against rescaled dimenions.}
%\label{fig:MultivariateARCH}
%\end{figure}
%
%We see from Fig. \ref{fig:MultivariateARCH} that the lasso estimates behave exactly as theory predicts even in nonlinear model!
\end{exmp}

